Deterministic enumeration of all minimum cut-sets and $k$-cut-sets in hypergraphs for fixed $k$

We consider the problem of deterministically enumerating all minimum $k$-cut-sets in a given hypergraph for any fixed $k$. The input here is a hypergraph $G = (V, E)$ with non-negative hyperedge costs. A subset $F$ of hyperedges is a $k$-cut-set if the number of connected components in $G - F$ is at least $k$ and it is a minimum $k$-cut-set if it has the least cost among all $k$-cut-sets. For fixed $k$, we call the problem of finding a minimum $k$-cut-set as Hypergraph-$k$-Cut and the problem of enumerating all minimum $k$-cut-sets as Enum-Hypergraph-$k$-Cut. The special cases of Hypergraph-$k$-Cut and Enum-Hypergraph-$k$-Cut restricted to graph inputs are well-known to be solvable in (randomized as well as deterministic) polynomial time. In contrast, it is only recently that polynomial-time algorithms for Hypergraph-$k$-Cut were developed. The randomized polynomial-time algorithm for Hypergraph-$k$-Cut that was designed in 2018 (Chandrasekaran, Xu, and Yu, SODA 2018) showed that the number of minimum $k$-cut-sets in a hypergraph is $O(n^{2k-2})$, where $n$ is the number of vertices in the input hypergraph, and that they can all be enumerated in randomized polynomial time, thus resolving Enum-Hypergraph-$k$-Cut in randomized polynomial time. A deterministic polynomial-time algorithm for Hypergraph-$k$-Cut was subsequently designed in 2020 (Chandrasekaran and Chekuri, FOCS 2020), but it is not guaranteed to enumerate all minimum $k$-cut-sets. In this work, we give the first deterministic polynomial-time algorithm to solve Enum-Hypergraph-$k$-Cut (this is non-trivial even for $k = 2$). Our algorithms are based on new structural results that allow for efficient recovery of all minimum $k$-cut-sets by solving minimum $(S,T)$-terminal cuts. Our techniques give new structural insights even for enumerating all minimum cut-sets (i.e., minimum 2-cut-sets) in a given hypergraph.

==> conclusion.tex <==
\section{Conclusion and Open Problems} 
\label{sec:conclusion}
\knote{This section will not go into the final version.}

Our work approaches global cut and partitioning problems via minimum $(S,T)$-terminal cuts. The questions below appear to be natural directions for understanding the power of this approach. In all these questions, we need an appropriate structural conjecture. 

\begin{enumerate}
    \item Can we achieve the tight upper bound of $O_k(n^k)$ on the number of minimum $k$-partitions in a connected graph via structural results? 
    \item Min-max hypergraph $k$-partition:
    \begin{enumerate}
        \item The number of optimum min-max graph $k$-partitions is $n^{O(k^2)}$. We do not know an example achieving this lower bound, so it is possible that the upper bound is $n^{O(k)}$. Can the upper bound be improved via structural results? 
        \item Can we bound the number of $k$-cut-sets that correspond to optimum min-max hypergraph $k$-partitions? 
    \end{enumerate}
    \item Can we solve multiobjective minimum cut in hypergraphs in polynomial time? 
    \begin{enumerate}
        \item Conjecture: Every $\alpha$-approximate min cut in a connected graph can be obtained as the source minimal minimum $(S, T)$-terminal cut for some subsets $S$ and $T$ of size $O(alpha)$. Can this be proved using one of the three proof techniques for Theorem \ref{theorem: structure thm 2-for-min-cut}? i.e., either via canonical decomposition or via the three-cut-set lemma or via Theorem \ref{theorem:hypergraph-uncrossing}? This conjecture will give an alternative efficient algorithm to solve multiobjective minimum cut in graphs. 
    \end{enumerate}
\end{enumerate}

\knote{Need to replace the recursive algorithm with a non recursive algorithm for the journal version. }


